Let GPT be a Math Tutor: Teaching Math Word Problem Solvers with Customized Exercise Generation

In this paper, we present a novel approach for distilling math word problem solving capabilities from large language models (LLMs) into smaller, more efficient student models. Our approach is designed to consider the student model's weaknesses and foster a tailored learning experience by generating targeted exercises aligned with educational science principles, such as knowledge tracing and personalized learning. Concretely, we let GPT-3 be a math tutor and run two steps iteratively: 1) assessing the student model's current learning status on a GPT-generated exercise book, and 2) improving the student model by training it with tailored exercise samples generated by GPT-3. Experimental results reveal that our approach outperforms LLMs (e.g., GPT-3 and PaLM) in accuracy across three distinct benchmarks while employing significantly fewer parameters. Furthermore, we provide a comprehensive analysis of the various components within our methodology to substantiate their efficacy.

==> tbl_case.tex <==
\begin{table*}
\small
\renewcommand\arraystretch{1.2}
\centering
\begin{tabular}{|p{1.6cm}|p{13.5cm}|}
\hline
\multicolumn{2}{|>{\columncolor{good_color}}c|}{\textbf{Good Generated Problem Cases}} \\
\hline
%\textbf{Source Problem Problem} & luke scored N0 points after playing N1 rounds of a trivia game and . if he gained the same number of points each round how many points did he score per round ?\\
%\hline
%\textbf{Answer} & N0 / N1\\
%\hline
\textbf{Source Problem} & In a school there are N0 girls and N1 boys . how many more girls than boys does the school have ?\\
\hline
\textbf{Answer} & N0 - N1\\
\hline
\textbf{Generated Problem} & In a zoo there are N0 lions and N1 tigers. How many more lions than tigers are there in the zoo?\\
\hline
\textbf{Answer} & N0 - N1\\
\hline
\textbf{Source Problem} & In a school there are N0 girls and N1 boys . N2 more girls joined the school . how many more girls than boys does the school have ?\\
\hline
\textbf{Answer} & N0 + N2 - N1\\
\hline
\textbf{Generated Problem} & In a school there are N0 girls and N1 boys. N2 more girls joined the school. How many girls are there in total now ?\\
\hline
\textbf{Answer} & N0 + N2\\
\hline
\multicolumn{2}{|>{\columncolor{bad_color}}c|}{\textbf{Bad Generated Problem Cases}} \\
\hline
\textbf{Source Problem} & For gwen's birthday she received N0 dollars. she spent some money and has N1 dollars left with her. how much money did she spend?\\
\hline
\textbf{Answer} & N0 - N1\\
\hline
\textbf{Generated Problem} & For gwen's birthday she received N0 dollars. she spent some money and now has N1 dollars left. How much money did she originally have?\\
\hline
\textbf{Answer} & N0 = N1 + spent amount (Wrong format)\\
\hline
\end{tabular}
\caption{Examples of good and bad problem generation cases.}
\label{tab:case}
\end{table*}
